TSSuBERT: Tweet Stream Summarization Using BERT

The development of deep neural networks and the emergence of pre-trained language models such as BERT allow to increase performance on many NLP tasks. However, these models do not meet the same popularity for tweet summarization, which can probably be explained by the lack of existing collections for training and evaluation. Our contribution in this paper is twofold : (1) we introduce a large dataset for Twitter event summarization, and (2) we propose a neural model to automatically summarize huge tweet streams. This extractive model combines in an original way pre-trained language models and vocabulary frequency-based representations to predict tweet salience. An additional advantage of the model is that it automatically adapts the size of the output summary according to the input tweet stream. We conducted experiments using two different Twitter collections, and promising results are observed in comparison with state-of-the-art baselines.

==> discussion.tex <==
\section{Results and Discussion}
\label{sec:disc}

We can see in Table~\ref{tab:evaluation_mycollection} that our model performs better for the ROUGE-1 and ROUGE-2. The score improvement is around 36\% and 27\% for ROUGE-1 F, 16\% and 10\% for ROUGE-2 F and -3\%, -2\% for the cosinus similarity with general embeddings respectively for micro and macro scores.
The improvements are statistically significant for ROUGE-1 and ROUGE-2 but not for COS Embeddings (Wilcoxon test, $p-value$<0.05\footnote{We did not use the Student t-test, the distribution was not Gaussian for all models using Shapiro-Wilk test.}).

We can see in Table~\ref{tab:evaluation_mycollection} that our model performs better for the ROUGE-1 and ROUGE-2. The score improvement is around 4\% and 3\% for ROUGE-1 F, 7\% and 7\% for ROUGE-2 F and -3\%, -1\% for the cosinus similarity with general embeddings respectively for micro and macro scores.
The improvements are statistically significant for ROUGE-1 and ROUGE-2 but not for COS Embeddings (Wilcoxon test, $p-value$<0.05\footnote{We did not use the Student t-test, the distribution was not Gaussian for all models using Shapiro-Wilk test.}).

We can see in Table~\ref{tab:evaluation} that our model performs better for the 3 evaluated metrics. The scores improvement is around 9\% for ROUGE-1 F, 32\% for ROUGE-2 F and 3\% for the cosinus similarity with general embeddings. The improvements are statistically significant (Wilcoxon test, $p-value$<0.05\footnote{We did not use the Student t-test, the distribution was not Gaussian for all models using Shapiro-Wilk test.}).

Beyond the better scores, these results are very promising for further improvements. These results show that neural models could find features itself to predict a relevant score to be or not in a summary. Moreover, we think our model can be upgrade easily.

\subsection{Effects of the addition of the tokens frequency}

We first built a model without the tokens frequency part. However, for the test evaluation, in two third cases the model predicted only 0.0 relevance scores. By adding the tokens frequency we gain in stability of the model.
